Hairy black holes and other compact objects in theories of gravity

In the realm of spacetimes governed by Einstein's general relativity and containing only Maxwell's electromagnetic field, stationary black holes are fully characterized by their mass, electric or magnetic charge, and angular momentum -- a property encapsulated in a version of the no-hair theorem. However, the validity of this theorem is contingent on certain assumptions, and when these are relaxed, new solutions describing hairy black holes arise. To date, astronomical observations have not provided concrete evidence of any type of black hole hair. Nevertheless, the development of increasingly precise gravitational wave detectors has sparked renewed interest in hairy black holes. In this thesis, we delve into two approaches to circumvent the no-hair theorem. The first option consists in describing the spacetime metric by an alternative theory of gravitation. We investigate the dynamical stability of hairy black holes in a vacuum spacetime described by the theory of massive bigravity. We show that hairy black holes in bigravity can describe both stellar black holes and supermassive black holes. The second approach is to keep Einstein's equations but to consider a different material content than Maxwell's electromagnetic field. For this we choose the fields of the electroweak theory. In the absence of gravitation, this theory describes magnetic monopoles with infinite mass. General relativity allows for their regularization by concealing their Coulombian singularity within an event horizon. After providing a detailed analysis of the internal structure of monopoles in flat space, we investigate how their properties generalize to the black hole case. Lastly, we study a particular example of soliton -- boson stars -- arising when a complex scalar field is coupled to general relativity. We construct chains of boson stars by solving the elliptic field equations using the finite element method.

==> olf_4th_couv.tex <==
%auto-ignore
\thispagestyle{empty}
    \newgeometry{top=0.5cm,bottom=0.5cm,left=1.2cm,right=1.2cm}

    \hspace{-0.7cm}
	\includegraphics[width=0.3\textwidth]{Logo/logo_univtours}
    \hfill
    \includegraphics[width=0.22\textwidth]{Logo/INSA_CVL.png}
    \hfill
	\includegraphics[width=0.2\textwidth]{Logo/logo_univorleans}\\
    \vspace{-0.5cm}
    {
    \fontsize{10pt}{12pt}\selectfont
    \section*{R\'esum\'e}
	

    Dans le cadre d’un espace-temps décrit par la relativité générale d’Einstein, sur lequel évolue uniquement le champ électromagnétique de Maxwell, les trous noirs stationnaires sont complètement caractérisés par leur masse, leur charge électrique ou magnétique, et leur moment cinétique : il s'agit de l'une des versions du théorème de calvitie. Pour autant, lorsque certaines des hypothèses de ce théorème sont omises, il a été établi qu'il cesse de s’appliquer. Cela conduit à l’émergence de trous noirs dits chevelus. Jusqu'à présent, les observations astronomiques ne permettent pas de détecter les «~cheveux~» des trous noirs. Cependant, avec le développement de détecteurs d'ondes gravitationnelles toujours plus précis, les trous noirs chevelus restent un sujet d'étude important en physique théorique. Dans cette thèse, nous considérons deux options permettant de s'affranchir du théorème de calvitie.

    La première option consiste à décrire la métrique de l’espace-temps par une théorie de gravitation alternative. Nous étudierons la stabilité de trous noirs chevelus dans un espace-temps vide décrit par la théorie de la bigravité massive. Cette théorie est connue pour ses solutions cosmologiques permettant de décrire un Univers en expansion accélérée sans avoir besoin de recourir à la constante cosmologique. Nous montrerons que les trous noirs chevelus en bigravité, obtenus à l’aide de méthodes numériques, sont capables de représenter tant des trous noirs stellaires que des trous noirs supermassifs.

    Une autre possibilité est de garder les équations d’Einstein, mais de considérer un contenu matériel autre que le champ électromagnétique de Maxwell. Nous choisirons pour cela les champs de la théorie électrofaible. Lorsque la gravitation est omise, cette théorie décrit des monopôles magnétiques de masse infinie. La relativité générale permet de les régulariser en masquant leur singularité coulombienne derrière un horizon des évènements. Les monopôles deviennent alors des trous noirs chargés magnétiquement, pouvant être chevelus. Ces trous noirs électrofaibles pourraient s'être formés lors de fluctuations primordiales, aux tout premiers instants de l’Univers. Après avoir étudié en détail la structure interne des monopôles en espace-temps plat, nous verrons comment leurs propriétés se généralisent au cas gravitationnel.

    Lorsqu’un trou noir chevelu voit le rayon de son horizon se réduire à zéro, les champs externes restent, et la configuration ainsi obtenue est appelée un soliton. Nous étudierons pour terminer un cas particulier de soliton obtenu lorsqu’un champ scalaire complexe est couplé à la relativité générale. Nous construirons des chaînes de ces solitons, appelés étoiles à bosons. Les équations aux dérivées partielles sous-jacentes seront résolues à l’aide de la méthode des éléments finis : une approche originale et peu utilisée par la communauté de la relativité numérique.

    \vspace{0.2cm}
    \textbf{Mots-clés : } trous noirs, gravité massive, méthodes numériques, monopôles magnétiques, théorie des champs classiques, relativité numérique.


    \section*{Abstract}
	
	In the realm of spacetimes governed by Einstein's general relativity and containing only Maxwell's electromagnetic field, stationary black holes are fully characterized by their mass, electric or magnetic charge, and angular momentum -- a property encapsulated in a version of the no-hair theorem. However, the validity of this theorem is contingent on certain assumptions, and when these are relaxed, it has been established that the theorem does not always apply. This gives rise to the so-called hairy black holes. To date, astronomical observations have not provided concrete evidence of any type of black hole "hair". Nevertheless, the development of increasingly precise gravitational wave detectors has sparked renewed interest in hairy black holes. In this thesis, we delve into two approaches to circumvent the no-hair theorem.

    The first option consists in describing the spacetime metric by an alternative theory of gravitation. We investigate the dynamical stability of hairy black holes in a vacuum spacetime described by the theory of massive bigravity. This theory is known for its cosmological solutions which can account for a self-accelerating expansion of the Universe without requiring the use of the cosmological constant. We show that hairy black holes in bigravity, which are obtained using numerical methods, can describe both stellar black holes and supermassive black holes.

    Another approach is to keep Einstein's equations but to consider a different material content than Maxwell's electromagnetic field. For this we choose the fields of the electroweak theory. In the absence of gravitation, this theory describes magnetic monopoles with infinite mass. General relativity allows for their regularization by concealing their Coulombian singularity within an event horizon. As a result, monopoles become magnetically charged black holes which can exhibit a non-Abelian hair. These electroweak black holes might have formed during primordial fluctuations in the early Universe. After providing a detailed analysis of the internal structure of monopoles in flat space, we investigate how their properties generalize to the black hole case.

    When the horizon radius of a hairy black hole shrinks to zero, only its external fields remain, giving rise to a configuration known as a soliton. Lastly, we study a particular example of soliton that arises when a complex scalar field is coupled to general relativity. We construct chains of these solitons, which are referred to as boson stars, by solving the underlying partial differential equations using the finite element method. This technique is not very common in the numerical relativity community and provides an alternative to the finite difference method.

    \vspace{0.2cm}
    \textbf{Keywords: } black holes, massive gravity, numerical methods, magnetic monopoles, classical field theory, numerical relativity.
    \vfill
    }


==> pdg.tex <==
%auto-ignore
%\usepackage{geometry}

\makeatletter

\def\@specialite{Spécialité}
\newcommand{\specialite}[1]{
	\def\@specialite{#1}
}

\def\@directeur{directeur}
\newcommand{\directeur}[1]{
	\def\@directeur{#1}
}

\def\@encadrant{encadrant}
\newcommand{\encadrant}[1]{
	\def\@encadrant{#1}
}

\def\@president{}{}
\newcommand{\president}[2]{
	\def\@president{#1	(\textit{Président du jury}) & #2\\}
    %\def\@president{#1 & #2\\}
}

\def\@rapporteura{}{}
\newcommand{\rapporteura}[2]{
	\def\@rapporteura{#1	& #2\\}
}

\def\@rapporteurb{}{}
\newcommand{\rapporteurb}[2]{
	\def\@rapporteurb{#1	& #2\\}
}

\def\@rapporteurc{}{}
\newcommand{\rapporteurc}[2]{
	\def\@rapporteurc{#1	& #2\\}
}

\def\@jurya{}{}
\newcommand{\jurya}[2]{
	\def\@jurya{#1	& #2\\}
}

\def\@juryb{}{}
\newcommand{\juryb}[2]{
	\def\@juryb{#1	& #2\\}
}

\def\@juryc{}{}
\newcommand{\juryc}[2]{
	\def\@juryc{#1	& #2\\}
}

\def\@juryd{}{}
\newcommand{\juryd}[2]{
	\def\@juryd{#1	& #2\\}
}

\def\@jurye{}{}
\newcommand{\jurye}[2]{
	\def\@jurye{#1	& #2\\}
}

\def\@juryf{}{}
\newcommand{\juryf}[2]{
	\def\@juryf{#1	& #2\\}
}

\makeatother

\makeatletter
\newcommand{\pagedegarde}{
	\newgeometry{top=1cm, bottom=1cm, left=1cm, right=1cm}
	%\AddToShipoutPicture*{\BackgroundPic}
	%\AddToShipoutPicture*{\EtiquetteThese}
	\begin{titlepage}
		\centering
		\includegraphics[width=0.3\textwidth]{Logo/logo_univtours}
        \hfill
        \includegraphics[width=0.22\textwidth]{Logo/INSA_CVL.png}
		\hfill
		\includegraphics[width=0.2\textwidth]{Logo/logo_univorleans}\\
		\vspace{1cm}
		{\LARGE \textbf{UNIVERSITÉ DE TOURS}}\\
		\vspace{1cm}
		{\Large \bfseries ÉCOLE DOCTORALE : \textit{MIPTIS}}\\[10pt]
		{\Large \bfseries Institut Denis Poisson}\\
		\vspace{1cm}
		{\huge \bfseries TH\`{E}SE} \ {\large présentée par :} \\[10pt]
		{\Large \bfseries \@author} \\[10pt]
		{\large soutenue le :} {\large \bfseries \@date} \\
		{\vspace{1cm}}
		{\large pour obtenir le grade de :} {\large \bfseries Docteur de l'université de Tours} \\[10pt]
		{\large Discipline/Spécialité : \@specialite} \\
		{\vspace{1cm}}
		{
			%\renewcommand{\arraystretch}{1}
			\setlength{\tabcolsep}{0.4cm}
			\begin{tabular}{|p{14cm}|}
				\hline
				\Large \bfseries \begin{center} \@title \end{center} \\
				\hline
			\end{tabular}
		} \\
		{\vspace{1cm}}
		{\large Directeur de thèse :} {\large \bfseries \@directeur}\\
		{\large Co-encadrant de thèse :} {\large \bfseries \@encadrant}\\
		\vspace{0.5cm}
		\rule{\linewidth}{0.5mm}
		{\begin{center} \large \bfseries Rapporteurs \end{center}}
		\begin{tabular}{lll}
			\@rapporteura
			\@rapporteurb
		\end{tabular}
		
		{\begin{center} \large \bfseries Jury \end{center}}
		\begin{tabular}{lll}
			\@jurya
            \@president
            \@jurye
			\@juryb
            \@juryf
            \@juryc
            \@juryd
		\end{tabular}
		%\vfill
	\end{titlepage}
	
	
	
	
	\restoregeometry  
}

